Dataset and Baseline System for Multi-lingual Extraction and Normalization of Temporal and Numerical Expressions

Temporal and numerical expression understanding is of great importance in many downstream Natural Language Processing (NLP) and Information Retrieval (IR) tasks. However, much previous work covers only a few sub-types and focuses only on entity extraction, which severely limits the usability of identified mentions. In order for such entities to be useful in downstream scenarios, coverage and granularity of sub-types are important; and, even more so, providing resolution into concrete values that can be manipulated. Furthermore, most previous work addresses only a handful of languages. Here we describe a multi-lingual evaluation dataset - NTX - covering diverse temporal and numerical expressions across 14 languages and covering extraction, normalization, and resolution. Along with the dataset we provide a robust rule-based system as a strong baseline for comparisons against other models to be evaluated in this dataset. Data and code are available at \url{https://aka.ms/NTX}.

==> data_dist.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[t]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}ccccccccccccccc@{}}
% \toprule
%                 & Arabic & Chinese & Dutch & English & French & German & Hindi & Italian & Japanese & Korean & Portuguese                                        & Spanish & Swedish                                            & Turkish \\ \midrule
% Cardinal        & 284    & 362     & 162   & 233     & 273    & 55     & 192   & 152     & 764      & 254    & 174                                               & 206     & 152                                                & 129     \\
% Number Range    & 145    & 65      & 53    & 87      & 85     & 6      & 76    & 34      & 185      & 132    &  50 & 98      & 30  & 61      \\
% Ordinal         & 70     & 7       & 48    & 54      & 70     & 38     & 64    & 31      & 101      & 68     & 33                                                & 82      & 43                                                 & 39      \\
% Percentage      & 27     & 152     & 13    & 20      & 35     & 15     & 16    & 11      & 204      & 30     & 51                                                & 66      & 11                                                 & 11      \\
% Age             & 0      & 10      & 17    & 19      & 18     & 14     & 21    & 15      & 18       & 19     & 18                                                & 18      & 20                                                 & 18      \\
% Currency        & 0      & 35      & 32    & 180     & 114    & 39     & 115   & 104     & 68       & 108    & 124                                               & 122     & 36                                                 & 109     \\
% Dimension       & 0      & 36      & 74    & 93      & 60     & 28     & 53    & 55      & 64       & 64     & 65                                                & 54      & 67                                                 & 56      \\
% Temperature     & 0      & 10      & 34    & 36      & 41     & 12     & 45    & 34      & 38       & 38     & 47                                                & 45      & 35                                                 & 34      \\
% Phone Number    &        & 391     &       & 405     &        &        &       &         &          &        & 85                                                &         &                                                    &         \\\bottomrule
% \end{tabular}}
% \end{table*}



% \begin{table*}[t]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}ccccccccccccccc@{}}
% \toprule
%                 & Arabic & Chinese & Dutch & English & French & German & Hindi & Italian & Japanese & Korean & Portuguese                                        & Spanish & Swedish                                            & Turkish \\ \midrule
% Date            & 118    & 64      & 226   & 148     & 228    & 28     & 122   & 107     & 214      & 194    & 65                                                & 73      & 132                                                & 94      \\
% Date Range      & 305    & 67      & 319   & 352     & 514    & 63     & 318   & 241     & 246      & 180    & 60                                                & 374     & 60  & 221     \\
% DateTime        & 72     & 15      & 134   & 81      & 125    & 21     & 67    & 68      & 87       & 59     & 61                                                & 63      & 15  & 64      \\
% DateTime Range  & 73     & 27      & 180   & 96      & 183    & 32     & 86    & 77      & 99       & 62     & 41                                                & 118     & 27  & 67      \\
% Model - Overall & 112    & 257     & 741   & 916     & 884    & 202    & 507   & 114     & 584      & 316    & 156                                               & 825     & 112 & 316     \\
% Duration        & 55     & 15      & 87    & 62      & 103    & 21     & 61    & 44      & 44       & 34     & 21                                                & 23      & 15  & 33      \\
% Holiday         & 18     & 35      & 46    & 26      & 50     & 61     & 30    & 11      & 43       & 15     & 14                                                & 17      & 11  & 19      \\
% Set             & 27     & 8       & 52    & 32      & 58     & 13     & 30    & 27      & 33       & 27     & 20                                                & 18      & 8   & 25      \\
% Time            & 74     & 14      & 138   & 93      & 198    & 26     & 84    & 67      & 79       & 61     & 58                                                & 56      & 14  & 69      \\
% Time Range      & 55     & 16      & 122   & 65      & 109    & 13     & 63    & 52      & 67       & 56     & 30                                                & 93      & 13  & 54      \\
% Timezone        & 0      & 0       & 19    & 49      & 48     & 0      & 0     & 0       & 0        & 0      & 0                                                 & 0       & 54                                                 & 0       \\ \bottomrule
% \end{tabular}}
% \end{table*}


\begin{table*}[t]
\small\centering
%\resizebox{\textwidth}{!}{
\begin{tabular}{clcccccccccccccc}
\toprule
& &\multicolumn{14}{c}{Language} \\
          &     &  \rotr{Arabic} & \rotr{Chinese} & \rotr{Dutch} & \rotr{English} & \rotr{French} & \rotr{German} & \rotr{Hindi} & \rotr{Italian} & \rotr{Japanese} & \rotr{Korean} & \rotr{Portuguese}                                        & \rotr{Spanish} & \rotr{Swedish}                                            & \rotr{Turkish} \\ \midrule
               \multirow{9}{*}{\rotrow{Sub-type}}
&Cardinal        & 284    & 362     & 162   & 233     & 273    & 55     & 192   & 152     & 764      & 254    & 174                                               & 206     & 152                                                & 129     \\
&Number Range    & 145    & 65      & 53    & 87      & 85     & 6      & 76    & 34      & 185      & 132    &  50 & 98      & 30  & 61      \\
& Ordinal         & 70     & 7       & 48    & 54      & 70     & 38     & 64    & 31      & 101      & 68     & 33                                                & 82      & 43                                                 & 39      \\
&Percentage      & 27     & 152     & 13    & 20      & 35     & 15     & 16    & 11      & 204      & 30     & 51                                                & 66      & 11                                                 & 11      \\
&Age             & 0      & 10      & 17    & 19      & 18     & 14     & 21    & 15      & 18       & 19     & 18                                                & 18      & 20                                                 & 18      \\
&Currency        & 0      & 35      & 32    & 180     & 114    & 39     & 115   & 104     & 68       & 108    & 124                                               & 122     & 36                                                 & 109     \\
&Dimension       & 0      & 36      & 74    & 93      & 60     & 28     & 53    & 55      & 64       & 64     & 65                                                & 54      & 67                                                 & 56      \\
&Temperature     & 0      & 10      & 34    & 36      & 41     & 12     & 45    & 34      & 38       & 38     & 47                                                & 45      & 35                                                 & 34      \\
&Phone Number    &        & 391     &       & 405     &        &        &       &         &          &        & 85                                                &         &                                                    &         \\\bottomrule
\end{tabular}%}
\caption{Numbers of numerical entities by language and sub-type.}
\end{table*}



\begin{table*}[t]
%\resizebox{\textwidth}{!}{
\small\centering
\begin{tabular}{clcccccccccccccc}
	\toprule
	& &\multicolumn{14}{c}{Language} \\
	&     &  \rotr{Arabic} & \rotr{Chinese} & \rotr{Dutch} & \rotr{English} & \rotr{French} & \rotr{German} & \rotr{Hindi} & \rotr{Italian} & \rotr{Japanese} & \rotr{Korean} & \rotr{Portuguese}                                        & \rotr{Spanish} & \rotr{Swedish}                                            & \rotr{Turkish} \\ \midrule
	\multirow{9}{*}{\rotrow{Sub-type}}
&Date            & 118    & 64      & 226   & 148     & 228    & 28     & 122   & 107     & 214      & 194    & 65                                                & 73      & 132                                                & 94      \\
&Date Range      & 305    & 67      & 319   & 352     & 514    & 63     & 318   & 241     & 246      & 180    & 60                                                & 374     & 60  & 221     \\
&DateTime        & 72     & 15      & 134   & 81      & 125    & 21     & 67    & 68      & 87       & 59     & 61                                                & 63      & 15  & 64      \\
&DateTime Range  & 73     & 27      & 180   & 96      & 183    & 32     & 86    & 77      & 99       & 62     & 41                                                & 118     & 27  & 67      \\
&Model - Overall & 112    & 257     & 741   & 916     & 884    & 202    & 507   & 114     & 584      & 316    & 156                                               & 825     & 112 & 316     \\
&Duration        & 55     & 15      & 87    & 62      & 103    & 21     & 61    & 44      & 44       & 34     & 21                                                & 23      & 15  & 33      \\
&Holiday         & 18     & 35      & 46    & 26      & 50     & 61     & 30    & 11      & 43       & 15     & 14                                                & 17      & 11  & 19      \\
&Set             & 27     & 8       & 52    & 32      & 58     & 13     & 30    & 27      & 33       & 27     & 20                                                & 18      & 8   & 25      \\
&Time            & 74     & 14      & 138   & 93      & 198    & 26     & 84    & 67      & 79       & 61     & 58                                                & 56      & 14  & 69      \\
&Time Range      & 55     & 16      & 122   & 65      & 109    & 13     & 63    & 52      & 67       & 56     & 30                                                & 93      & 13  & 54      \\
&Timezone        & 0      & 0       & 19    & 49      & 48     & 0      & 0     & 0       & 0        & 0      & 0                                                 & 0       & 54                                                 & 0       \\ \bottomrule
\end{tabular}%}
\caption{Numbers of temporal entities by language and sub-type.}
\end{table*}
